ZeroGen: Efficient Zero-shot Learning via Dataset Generation

There is a growing interest in dataset generation recently due to the superior generative capacity of large pre-trained language models (PLMs). In this paper, we study a flexible and efficient zero-short learning method, \textsc{ZeroGen}. Given a zero-shot task, we first generate a dataset from scratch using PLMs in an unsupervised manner. Then, we train a tiny task model (e.g., LSTM) under the supervision of the synthesized dataset. This approach allows highly efficient inference as the final task model only has orders of magnitude fewer parameters comparing to PLMs (e.g., GPT2-XL). Apart from being annotation-free and efficient, we argue that \textsc{ZeroGen} can also provide useful insights from the perspective of data-free model-agnostic knowledge distillation, and unreferenced text generation evaluation. Experiments and analysis on different NLP tasks, namely, text classification, question answering, and natural language inference, show the effectiveness of \textsc{ZeroGen}.

==> Zero-shot Learning via Unsupervised Dataset Generation (2)/tabs/data_scale.tex <==
% \begin{table}[t]
% \scalebox{0.75}{
% \begin{tabular}{lll|ccc}
% \toprule
% \multicolumn{1}{c}{\textbf{Setting}} & \textbf{TAM} & \textbf{Scale} & \textbf{IMDB} & \textbf{SQuAD} & \textbf{QNLI} \\
% \hline
% \multirow{2}{*}{\textit{\textsc{Supervised}}} & LSTM & 1x & 84.60 & 41.86/57.22 & 69.00 \\
%  & DistilBERT & 1x & 87.24 & 76.28/84.67 & 88.05 \\
%  \hline
% \textit{\textsc{Prompting}} & - & 0x & 80.64 & 4.61/13.32 & 60.60 \\
% \hline
% \multirow{6}{*}{\textit{\textsc{ZeroGen}}} & \multirow{3}{*}{LSTM} & 0.5x & 53.20 & \textbf{7.71}/12.11 & 52.39 \\
%  &  & 1x & 59.30 & \textbf{8.57}/\textbf{13.63} & 51.16 \\
%  &  & 2x & 69.10 & \textbf{9.73}/\textbf{15.12} & 51.22 \\
%  \cline{2-6}
%  & \multirow{3}{*}{DistilBERT} & 0.5x & 80.05 & \textbf{20.47}/\textbf{27.20} & \textbf{69.80} \\
%  &  & 1x & \textbf{80.90} & \textbf{23.63}/\textbf{29.95} & \textbf{70.55} \\
%  &  & 2x & \textbf{81.60} & \textbf{25.25}/\textbf{31.50} & \textbf{71.19} \\
%  \bottomrule
% \end{tabular}}
% \caption{Comparison of different scale of synthetic dataset. We use GPT2-XL as the PLM for both \textsc{Prompting} and \textsc{ZeroGen} frameworks. }
% \label{tab:scale}
% \end{table}

\begin{table}[t]
\centering
\scalebox{0.7}{
\begin{tabular}{lll|ccc}
\toprule
\multicolumn{1}{c}{\textbf{Setting}} & \textbf{TAM} & \textbf{Scale} & \textbf{IMDB} & \textbf{SQuAD} & \textbf{QNLI} \\
\hline
\multirow{2}{*}{\textit{\textsc{Supervised}}} & LSTM & 1x & 84.60 & 41.86/57.22 & 69.00 \\
 & DistilBERT & 1x & 87.24 & 76.28/84.67 & 88.05 \\
 \hline
\textit{\textsc{Prompting}} & - & 0x & 80.64 & 4.61/13.32 & 60.60 \\
\hline
\multirow{6}{*}{\textit{\textsc{ZeroGen}}} & \multirow{3}{*}{LSTM} & 0.5x & 53.20 & \cc {7.71}/12.11 & {50.05} \\
 &  & 1x & 59.30 & \cc {8.57}/{13.63} & 51.16 \\
 &  & 2x & \textbf{69.10} & \cc \textbf{9.73}/\textbf{15.12} & \textbf{52.26} \\
 \cline{2-6}
 & \multirow{3}{*}{DistilBERT} & 0.5x & 80.05 & \cc {20.47}/{27.20} & \cc {69.80} \\
 &  & 1x & \cc {80.90} & \cc {23.63}/{29.95} & \cc {70.55} \\
 &  & 2x & \cc \textbf{81.60} & \cc \textbf{25.25}/\textbf{31.50} & \cc \textbf{71.19} \\
 \bottomrule
\end{tabular}}
\caption{Comparison of different scale of synthetic dataset. We use GPT2-XL as the PLM for both \textsc{Prompting} and \textsc{ZeroGen} frameworks. Under different scales of dataset, best results are \textbf{bolded}.}
\label{tab:scale}
\end{table}

==> Zero-shot Learning via Unsupervised Dataset Generation (2)/tabs/decoding.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[t]
\centering
\scalebox{0.75}{
% \begin{tabular}{ll|ccc}
% \toprule
% \multicolumn{1}{c}{\textbf{Setting}} & \textbf{Strategy} & \textbf{IMDb} & \textbf{SQuAD} & \textbf{QNLI} \\
% \hline
% \textit{\textsc{Prompting}} & - & 80.64 &  4.61/13.32 & 60.60 \\
% \hline
% \multirow{5}{*}{\textit{\textsc{ZeroGen}}} & Greedy & 54.70 & \cc 10.76/16.24 & 53.14 \\
%  & Top-k=5 & 57.30 & \cc \textbf{13.22/19.45} & \textbf{54.68} \\
%  & Top-k=40 & \textbf{72.24} & \cc 10.11/15.56 & 51.24 \\
%  & Top-k=80 & 71.10 & \cc 9.63/14.70 & 51.38 \\
%  & Nucleus p=0.9 & 71.80 & \cc 8.83/13.89 & 51.16 \\
%  \bottomrule
% \end{tabular}}

% \begin{tabular}{l|ccc}
% \toprule
% \textbf{Strategy} & \textbf{IMDb} & \textbf{SQuAD} & \textbf{QNLI} \\
% \hline
%  Greedy & 54.70 &  10.76/16.24 & 53.14 \\
%  Top-k=5 & 57.30 &  \textbf{13.22/19.45} & \textbf{54.68} \\
%  Top-k=40 & \textbf{72.24} &  10.11/15.56 & 51.24 \\
%  Top-k=80 & 71.10 &  9.63/14.70 & 51.38 \\
%  Nucleus p=0.9 & 71.80 &  8.83/13.89 & 51.16 \\
%  \bottomrule
% \end{tabular}}

\begin{tabular}{ll|ccc}
\toprule
\textbf{TAM} & \textbf{Strategy} & \textbf{IMDb} & \textbf{SQuAD} & \textbf{QNLI} \\
\hline
\multirow{5}{*}{DistilBERT} & Greedy & 74.40 & 24.19/31.16 & 63.59 \\
 & Top k=5 & 79.50 & \textbf{25.68/32.32} & \textbf{71.83} \\
 & Top k=40 & \textbf{83.70} & 24.70/31.21 & 70.40 \\
 & Top k=80 & \textbf{83.70} & 24.14/30.89 & 69.83 \\
 & Nucleus p=0.9 & 83.40 & 23.93/30.62 & 70.55 \\
 \hline
\multirow{5}{*}{LSTM} & Greedy & 54.70 & 10.76/16.24 & 53.14 \\
 & Top k=5 & 57.30 & \textbf{13.22/19.45} & \textbf{54.68} \\
 & Top k=40 & \textbf{72.24} & 10.11/15.56 & 51.24 \\
 & Top k=80 & 71.10 & 9.63/14.70 & 51.38 \\
 & Nucleus p=0.9 & 71.80 & 8.83/13.89 & 51.16 \\
 \bottomrule
\end{tabular}}

\caption{Results for comparing different decoding methods with selected parameters of each method. The best result under different decoding methods is \textbf{bolded}.
% \tao{why grey color? why showing Prompting results (may mislead inattentive reviewers)? why LSTM here and DBERT in Fig 2?}\yjc{we have a footnote to say that we observed similar trends when using DistilBERT, would it be redundant to include DistilBERT?}
}
\label{tab:decode}
\vspace{-3mm}
\end{table}

==> Zero-shot Learning via Unsupervised Dataset Generation (2)/tabs/main_results.tex <==

\begin{table*}[t]
\centering
\scalebox{0.8}{
\begin{tabular}{ll|ll|cccccc}
\toprule
\textbf{PLM} & \textbf{TAM} & \textbf{\#Param} & \textbf{Setting} & \textbf{IMDb} & \textbf{SST-2} & \textbf{SQuAD} & \textbf{AdversarialQA} & \textbf{QNLI} & \textbf{RTE} \\
\hline
 \multirow{2}{*}{-} & DistilBERT & 66M & \multirow{2}{*}{{\textsc{Supervised}}} & 87.24 & 89.68 & 76.28/84.67 & 18.6/29.85 & 88.05 & 58.12 \\
 & LSTM & $\sim$7M &  & 84.60 & 76.30 & 41.86/57.22 & 5.37/11.86 & 69.00 & 54.87 \\
 \hline
\multirow{3}{*}{GPT2} & - & 117M & \textit{\textsc{Prompting}} & 51.52 & 52.52 & 0.80/4.93 & 0.37/2.58 & 50.60 & \textbf{52.70} \\
 & DistilBERT & 66M & \multirow{2}{*}{\textit{\textsc{ZeroGen}}} & \cc\textbf{73.24} & \cc\textbf{80.39} & \cc\textbf{16.44/21.83} & \cc\textbf{5.20/8.26} & \cc\textbf{55.32} & 50.54 \\
 & LSTM & $\sim$7M &  & \cc{69.60} & \cc{70.40} & \cc{4.94/8.53} & \cc{1.00/3.83} & \cc{51.03} & 49.10 \\
 \hline
\multirow{3}{*}{GPT2-Large} & - & 762M & \textit{\textsc{Prompting}} & 80.20 & \textbf{87.84} & 3.53/10.78 & 1.47/5.16 & 55.10 & 54.51 \\
 & DistilBERT & 66M & \multirow{2}{*}{\textit{\textsc{ZeroGen}}} & \cc\textbf{83.56} & 85.44 & \cc\textbf{23.87/29.82} & \cc\textbf{5.93/9.63} & \cc\textbf{69.32} & \cc\textbf{58.48}$^{*}$ \\
 & LSTM & $\sim$7M &  & 78.20 & 75.10 & \cc{8.01/12.77} & \cc{2.33/5.24} & 51.27 & \cc{56.68}$^{*}$ \\
 \hline
\multirow{3}{*}{GPT2-XL} & - & 1.5B & \textit{\textsc{Prompting}} & 80.64 & \textbf{89.22} & 4.61/13.32 & 2.13/6.30 & 60.60 & 57.04 \\
 & DistilBERT & 66M & \multirow{2}{*}{\textit{\textsc{ZeroGen}}} & \cc\textbf{84.28} &  {87.27} & \cc\textbf{25.50/31.53} & \cc\textbf{6.33/9.96} & \cc\textbf{71.19} & \cc\textbf{59.93}$^{*}$ \\
 & LSTM & $\sim$7M &  & 79.80 & 78.40$^{*}$ & \cc{12.35/18.66} & \cc{3.23/6.34} & 52.26 & \cc{58.85}$^{*}$ \\
 \bottomrule
\end{tabular}}
\caption{Evaluation results for \textsc{ZeroGen} framework at three  different scales of PLM and two different scales of TAM.
The \textsc{ZeroGen} results that outperform \textsc{Prompting} using the same PLM are in \hl{grey}, and the best result for each task using the same PLM is \textbf{bolded}. $^{*}$ indicates that the result of TAM under \textsc{ZeroGen} framework outperforms the same TAM under \textsc{Supervised} framework. Due to the architecture difference in LSTM-based models among different tasks, we calculate the average number of parameters (i.e., 7M).
}
\label{tab:main}
\end{table*}

==> Zero-shot Learning via Unsupervised Dataset Generation (2)/tabs/notation.tex <==

\begin{table*}[t]
\centering
\scalebox{0.8}{
\begin{tabular}{l|llp{10cm}}
\toprule
 & \textbf{Dataset} & \textbf{Dataset Generation} & \textbf{Example} \\ 
 \hline
\multirow{2}{*}{\textbf{TC}} & \multirow{2}{*}{$\{(X, y)\}$} & \multirow{2}{*}{$X \sim P(X|f_{prompt}(y))$} & $\operatorname{Des}(y)$: \{positive, negative\} \\
 &  &  & $f_{prompt}$: The movie review in <$\operatorname{Des}(y)$> sentiment is: " \\ 
 \hline
\multirow{2}{*}{\textbf{NLI}} & \multirow{2}{*}{$\{(P, H, y)\}$} & {\multirow{2}{*}{$H \sim P(H|f_{prompt}(y, P))$}} & $\operatorname{Des}(y)$: \{correct, wrong\} \\
 &  &  & $f_{prompt}$: "<$P$>"\textbackslash{}nBased on the above description, the following sentence is definitely <$\operatorname{Des}(y)$>: " \\ 
 \hline
\textbf{QA} & $\{(Q, C, A)\}$ & $Q\sim P(Q|f_{prompt}(C,A))$ & $f_{prompt}$: The context is: "<$Q$>" \textbackslash{}n"<$A$>" is the answer of the following question: " \\ 
\bottomrule
\end{tabular}}
\caption{Notation and example of dataset generation methods for three tasks with our \proposed\ framework. $\operatorname{Des}(y)$: description of label $y$.}
\label{tab:approach}
\end{table*}

==> Zero-shot Learning via Unsupervised Dataset Generation (2)/tabs/one_case.tex <==

\begin{table*}[t]
\centering
\scalebox{0.8}{
\begin{tabular}{p{1.1cm}|p{13.5cm}p{4cm}}
\toprule
\textbf{Task} & \textbf{Prompt} & \textbf{Sampled Generation}\\
\hline
\multirow{2}{*}{SST-2}
& The movie review in \textbf{positive} sentiment for movie "\textbf{The Spiderwick Chronicles (Movie)}" is: " & It's an action-adventure movie about a crime fighter who must face an even bigger foe, then the end of the world, all in a funny, attractive, and moving way. \\
\cline{2-3}
& The movie review in \textbf{negative} sentiment for movie "\textbf{Fist Fight}" is: " & The action scenes are laughable, the characters lack personality, and the plot is boring. \\
\hline
% & \makecell[l]{The movie review in positive sentiment for movie "\textbf{The Spiderwick Chronicles (Movie)}" is: \\ The movie review in negative sentiment for movie "\textbf{Fist Fight}" is: } 
% & \makecell[l]{It's an action-adventure movie about a crime fighter who must face an even bigger foe, then the end of the world, all in a funny, attractive, and moving way. \\ The action scenes are laughable, the characters lack personality, and the plot is boring. } \\ 
\multirow{2}{*}{QNLI}
& Information: "\textbf{In September 1695, Captain Henry Every, an English pirate on board the Fancy, reached the Straits of Bab-el-Mandeb, where he teamed up with five other pirate captains to make an attack on the Indian fleet making the annual voyage to Mocha.}" \textbackslash n Question (answer \textbf{in} above information): " & Why did each of these captains enter the Straits of Bab-el-Mandeb? \\
\cline{2-3}
& Information: "\textbf{Gaddafi remained the government's public face, with the identities of the other RCC members only being publicly revealed on 10 January 1970.}" \textbackslash n Question (answer \textbf{not in} above information): " & Was the financing received from the international revolution from Germany (4)? \\
\hline
\multirow{2}{*}{RTE}
& "\textbf{Today about 75\% of people live in cities or towns. Art and culture are an important part of France.}" \textbackslash n Based on the above description, the following sentence is definitely \textbf{correct}: "& Today about 75\% of people live in cities and towns. \\
\cline{2-3}
& "\textbf{There are four identified subtypes of Ebola virus. Three of the four have caused disease in humans: Ebola-Zaire, Ebola-Sudan, and Ebola-Ivory Coast. The fourth, Ebola-Reston, has caused disease in non-human primates, but not in humans.}" \textbackslash n Based on the above description, the following sentence is definitely \textbf{wrong}: "& The most recently documented case was a Sierra Leonean man who died in 2015. \\
\hline
\multirow{1}{*}{SQuAD}
& The context is: "\textbf{On the other hand, in his study on nine of \"the Bibles most widely in use in the English-speaking world\", Bible scholar Jason BeDuhn, Professor of Religious Studies at the Northern Arizona University, wrote: \u201cThe NW [New World Translation] emerges as the most accurate of the translations compared.\u201d Although the general public and many Bible scholars assume that the differences in the New World Translation are the result of religious bias on the part of its translators, BeDuhn stated: \u201cMost of the differences are due to the greater accuracy of the NW as a literal, conservative translation of the original expressions of the New Testament writers.\u201d He added however that the insertion of the name Jehovah in the New Testament \"violate[s] accuracy in favor of denominationally preferred expressions for God.}" \textbackslash n "\textbf{Jehovah}" is the answer to the following question: "& Who is the one and only true God ?
% & \makecell[l]{Information: "\textbf{In September 1695, Captain Henry Every, an English pirate on board the Fancy, reached the Straits of Bab-el-Mandeb, where he teamed up with five other pirate captains to make an attack on the Indian fleet making the annual voyage to Mocha.}" \textbackslash n Question (answer in above information): " \\ Information: "\textbf{Gaddafi remained the government's public face, with the identities of the other RCC members only being publicly revealed on 10 January 1970.}"\textbackslash n Question (answer not in above information): "} 
\\ 
\bottomrule
\end{tabular}}

\caption{Generated examples for each task. We omit the example for IMDb and Adversarial QA tasks since we use the exactly same prompt as SST-2 and SQuAD task, respectively. The input conditions in each prompt are \textbf{bolded}.}
\label{tab:examples}
\end{table*}

==> Zero-shot Learning via Unsupervised Dataset Generation (2)/tabs/prompt.tex <==

\begin{table*}[t]
\centering
\renewcommand\arraystretch{1.2}  
\scalebox{0.7}{
\begin{tabular}{lllllcc}
\toprule
\textbf{Setting} & \textbf{Id} & \textbf{Prompt}& \textbf{Label word} <Y>  & \textbf{Prompt Type} & \textbf{IMDb} & \textbf{SST-2} \\
\hline
\multirow{4}{*}{\textit{\textsc{Prompting}}} & $P_1$ 
& \makecell[l]{"<X>" \\It was <Y>} 
& great/terrible & - &51.32 & 51.83\\ 
\cline{2-7}
& $P_2$ 
& \makecell[l]{
<Y> Movie Review: "<X>"} 
& Positive/Negative & Control code & 60.36 & 52.75\\ 
\cline{2-7}
& $P_3$ 
& \makecell[l]{Task: Write a review for a <Y> movie.
\\
Review:  "<X>" } 
 & good/bad & \makecell[l]{Control code with \\ task description} & 54.20 & 53.50\\ 
\cline{2-7}
& $P_4$ 
& \makecell[l]{The movie review in <Y> sentiment is "<X>"} 
 & \multirow{2}{*}{positive/negative} & \multirow{2}{*}{Natural language style} & 80.64 & 89.22\\ 
& $P_5$ 
& \makecell[l]{The <Y> movie review is "<X>"} & & & 67.60 & 72.36 \\ 
\hline
\multirow{5}{*}{\textit{\textsc{ZeroGen}}} & $P_1^{'}$ &   \makecell[l]{It was a review for a <Y> movie: " }  & great/terrible  & - & \underline{79.36} & \underline{75.00} \\
\cline{2-7}
 & $P_2$ &   \makecell[l]{<Y> Movie Review: "} & Positive/Negative & Control code & \underline{60.88} & \underline{67.43} \\
\cline{2-7}
 & $P_3$ &   \makecell[l]{Task: Write a review for a <Y> movie.
 \\
 Review: " }  & good/bad & \makecell[l]{Control code with \\task specification} & 83.40 & 78.90\\
\cline{2-7}
 & $P_4$ &   \makecell[l]{The movie review in <Y> sentiment is: "} & \multirow{3}{*}{positive/negative} & \multirow{3}{*}{Natural language style} & 81.84 & 86.24 \\
 & $P_4^{'}$ &   \makecell[l]{The movie review in <Y> sentiment for movie "<C>" is: "}  & & & 83.40 & 86.35 \\
& $P_5$ &   \makecell[l]{The <Y> movie review is "} & & & 77.44 & 77.06 \\
\bottomrule
\end{tabular}}
\caption{Results for different prompts on IMDb and SST-2 dev sets. We use GPT2-XL as PLM and DistilBERT as TAM.
<X> and <C> represents the input sentence  and generated movie name respectively. 
% \tao{the movie name is also auto generated by PLM before prompting the PLM to generate reviews?}
$P^{'}$ represents minor revised version of $P$ for text generation. 
For \textsc{ZeroGen}, results are reported using 100k training samples. Scores in \underline{underline} are trained on 10k generated samples, since the prompt ($P_1^{'}$ \& $P_2$) is too weak and cannot generate 100k distinct samples.
% \tao{maybe the caption is too long? leave some details to a footnote?}\jh{revised}
}
\label{tab:promptdesign_sst}
\end{table*}

==> Zero-shot Learning via Unsupervised Dataset Generation (2)/tabs/prompt_addtional.tex <==
\begin{table*}[t]
\centering
\scalebox{0.7}{
\begin{tabular}{llllcc}
\toprule
\textbf{Setting} & \textbf{Id} & \textbf{Prompt} &\textbf{Prompt Type}& \textbf{SQuAD} & \textbf{AdversarialQA} \\
\hline
\multirow{5}{*}{\textit{\textsc{Prompting}}} & $P_1$ 
& \makecell[l]{ Context: "<C>"\textbackslash nQuestion: "<X>"\textbackslash nAnswer: "}& Control code & 2.69/10.90 & 1.33/5.61 \\ 
\cline{2-6}
& $P_2$ 
& \makecell[l]{Task: Generate an answer given the context and question.\\
\textbackslash nContext: "<C>"\textbackslash nQuestion: "<X>"\textbackslash nAnswer: "} & \makecell[l]{Control code with\\ task description}
& 3.81/12.1	& 1.60/5.89\\ 
\cline{2-6}
& $P_3$ 
& \makecell[l]{"<C>"\textbackslash n
The answer to the question "<X>" is: "} & \multirow{4}{*}{Natural language style}
& 4.41/12.60 &	2.00/5.78 \\ 
& $P_4$ 
& \makecell[l]{"<C>"\textbackslash nBased on the above description, the\\ answer to the question "<X>" is: "} 
&  & 6.33/15.49 &	2.27/6.71 \\ 
& $P_5$ 
& \makecell[l]{The context is: "<C>"\textbackslash nThe answer to the question "<X>" is: "} 
& & 4.61/13.32 &	2.13/6.30\\ 
\hline
 \multirow{5}{*}{\textit{\textsc{ZeroGen}}}
& $P_1^{'}$ 
& \makecell[l]{ Context: "<C>"\textbackslash nAnswer: "<Y>"\textbackslash nQuestion: "} 
& Control code & 9.96/9.62 & 2.87/5.33 \\ 
\cline{2-6}
& $P_2^{'}$ 
& \makecell[l]{Task: Generate a question given the context and answer.\\
\textbackslash nContext: "<C>"\textbackslash nAnswer: "<Y>"\textbackslash nQuestion: "}  & \makecell[l]{Control code with\\ task description}
& 5.84/8.70 & 2.77/5.21 \\ 
\cline{2-6}
& $P_3^{'}$ 
& \makecell[l]{"<C>"\textbackslash n"<Y>" is the answer to the question: "} & \multirow{5}{*}{Natural language style}
& 24.55/29.36 &	5.30/8.82 \\ 
& $P_4^{'}$ 
& \makecell[l]{"<C>"\textbackslash nBased on the above description, "<Y>" is the\\ answer to the question: "} 
& & 23.58/29.84 & 5.87/9.58  \\ 
& $P_5^{'}$ 
& \makecell[l]{The context is: "<C>"\textbackslash n"<Y>" is the answer to the following\\ question: "} 
&  &23.93/30.62 & 5.97/10.02  \\ 
\bottomrule
\vspace{1mm}
\end{tabular}}

\scalebox{0.7}{
\begin{tabular}{lllllc}
\toprule
\textbf{Setting} & \textbf{Id} & \textbf{Prompt} & \textbf{Label words} <Y> & \textbf{Prompt Type} &\textbf{QNLI}\\
\hline
\multirow{5}{*}{\textit{\textsc{Prompting}}} & $P_1$ 
& \makecell[l]{Context: "<X>"\textbackslash nQuestion (answer <Y> the context): "} 
& in/not in  & \multirow{2}{*}{Control code
}& 50.51\\ 
& $P_2$ 
& \makecell[l]{Information: "<X>"\textbackslash nQuestion (answer <Y> above information): "} 
&   in/not in & & 50.52\\ 
\cline{2-6}
& $P_3$ 
& \makecell[l]{"<X>"\textbackslash n Based on the above description, the following question is\\ \textsc{[L1]} and \textsc{[L2]} be answered: "} 
&  \makecell[l]{clear/not clear\\ can/can not} & \multirow{6}{*}{Natural language style} &60.42  \\ 
& $P_4$ 
& \makecell[l]{The context sentence is: "<X>"\textbackslash nThe question is: "<X>"\textbackslash n\\
The context sentence <Y> the answer to the question. \\} 
& \makecell[l]{contains/\\doesn't contain} & &60.61 \\ 
& $P_5$ 
& \makecell[l]{The context sentence is: "<X>"\textbackslash nThe context sentence <Y> the\\ answer to the following question.\textbackslash nThe question is: "<X>"
} 
& \makecell[l]{contains/\\doesn't contain} & &58.02 \\ 
\hline
 \multirow{6}{*}{\textit{\textsc{ZeroGen}}}
& $P_1$ 
& \makecell[l]{Context: "<X>"\textbackslash nQuestion (answer <Y> the context): "} 
& in/not in &\multirow{2}{*}{Control code
} & 69.82\\ 
& $P_2$ 
& \makecell[l]{Information: "<X>"\textbackslash nQuestion (answer <Y> above information): "} 
&   in/not in & & 70.55\\ 
\cline{2-6}
& $P_3$ 
& \makecell[l]{"<X>"\textbackslash n Based on the above description, the following question is\\ \textsc{[L1]} and \textsc{[L2]} be answered: "} 
&  \makecell[l]{clear/not clear\\ can/can not} & \multirow{4}{*}{Natural language style
} &53.71 \\ 
& $P_4^{'}$ 
& \makecell[l]{The context sentence is: "<X>"\textbackslash nThe context sentence <Y> the\\ answer to the following question.\textbackslash nThe question is: "<X>"} 
& \makecell[l]{contains/\\doesn't contain}  & & 55.65 \\ 
\bottomrule
\vspace{1mm}
\end{tabular}}
\scalebox{0.7}{
\begin{tabular}{lllllc}
\toprule
\textbf{Setting} & \textbf{Id} & \textbf{Prompt} & \textbf{Label words} <Y> & \textbf{Prompt Type}& \textbf{RTE}\\
\hline
\multirow{5}{*}{\textit{\textsc{Prompting}}} & $P_1$ 
& \makecell[l]{Task: Write two sentences have the <Y> meaning.\\
\textbackslash nThe first sentence: "<X>"\textbackslash nThe second sentence: "} 
& same/complete different & \makecell[l]{Control code with \\task description} & 52.71\\ 
\cline{2-6}
& $P_2$ 
& \makecell[l]{Based on the fact that "<X>", it is <Y> that: "} 
&   correct/not correct & \multirow{4}{*}{Natural language style}  & 51.26 \\ 
& $P_3$ 
& \makecell[l]{Suppose "<X>", we <Y>  infer that: "} 
&  \makecell[l]{can/ can not} & & 52.71  \\ 
& $P_4$ 
& \makecell[l]{The context is: "<X>"\textbackslash nBased on the context, it is <Y>  that: "} 
& correct/not correct & &54.51  \\ 
& $P_5$ 
& \makecell[l]{"<X>"\textbackslash nBased on the above description, the following sentence\\ is definitely <Y> : "} 
& correct/wrong & &57.04 \\ 
\midrule
\multirow{5}{*}{\textit{\textsc{ZeroGen}}} & $P_1$ 
& \makecell[l]{Task: Write two sentences have the <Y> meaning.\\
\textbackslash nThe first sentence: "<X>"\textbackslash nThe second sentence: "} 
& same/complete different & \makecell[l]{Control code with \\task description} & 47.29\\ 
\cline{2-6}
& $P_2$ 
& \makecell[l]{Based on the fact that "<X>", it is <Y> that: "} 
&   correct/not correct & \multirow{4}{*}{Natural language style}  & 57.76 \\ 
& $P_3$ 
& \makecell[l]{Suppose "<X>", we <Y>  infer that: "} 
&  \makecell[l]{can/ can not} &  &49.46 \\ 
& $P_4$ 
& \makecell[l]{The context is: "<X>"\textbackslash nBased on the context, it is <Y>  that: "} 
& correct/not correct &  &61.73 \\ 
& $P_5$ 
& \makecell[l]{"<X>"\textbackslash nBased on the above description, the following sentence\\ is definitely <Y> : "} 
& correct/wrong & & 62.82 \\ 
\bottomrule
\end{tabular}}
\caption{Results for different prompts on Question Answering and  Natural language Inference tasks. Results are reported on dev set. For Question Answering, "<C>" represents the input context, "<X>" represents the input question, "<Y>" represents the generated answer. "\textbackslash n" represents the newline symbol. $P^{'}$ represents minor revised version of $P$ for text generation.}
\label{tab:promptdesign_others}
\end{table*}


==> Zero-shot Learning via Unsupervised Dataset Generation (2)/tabs/quality.tex <==
\begin{table}[t]
\centering
\scalebox{0.85}{
\begin{tabular}{l|ccc}
\toprule
\multicolumn{4}{c}{\textbf{\textsc{Diversity}}} \\
\hline
% \hline
\textbf{Strategy} & \textbf{IMDb} & \textbf{SQuAD} & \textbf{QNLI} \\
\hline
Oracle & 0.30 & 0.14 & 0.14 \\
\hline
Greedy & 0.92 & 0.55 & 0.54 \\
Top-k=5 & 0.59 & 0.29 & 0.28 \\
Top-k=40 & \textbf{0.25} & 0.17 & \textbf{0.14} \\
Top-k=80 & 0.20 & 0.17 & 0.12 \\
Nucleus p=0.9 & 0.15 & \textbf{0.16} & {0.11} \\
\bottomrule
\end{tabular}}
\scalebox{0.85}{
\begin{tabular}{l|ccc}
\toprule
% \hline
\multicolumn{4}{c}{\textbf{\textsc{Correctness}}} \\
\hline
% \hline
\textbf{Strategy} & \textbf{IMDb} & \textbf{SQuAD} & \textbf{QNLI} \\
\hline
Oracle & 92.42 & 95.37 & 92.96 \\
\hline
Greedy & 99.67 & \textbf{31.07} & \textbf{83.18} \\
Top-k=5 & \textbf{94.46} & 18.74 & 74.03 \\
Top-k=40 & {84.91} & 14.57 & 64.31 \\
Top-k=80 & 84.11 & 13.74 & 62.94 \\
Nucleus p=0.9 & 82.53 & {13.30} & {63.37} \\
\bottomrule
\end{tabular}}

\caption{Diversity and Correctness evaluation of generated datasets under different decoding strategies for each task. 
Oracle refers to the standard dataset with human annotations. 
Diversity is measured by Self-BLEU4, while Correctness is measured by a well-trained RoBERTa-Large model with standard dataset of each task.
% \tao{i assume this table is not complete yet. 
% ``the standard dataset'' means original human annotated dataset?
% why Self-BLEU4? maybe cite some other papers that also Self-BLEU4 to measure Diversity?
% a general q: other factors (e.g., PLM sizes and prompts, not just different decoding strategies) might affect data quality.
% why focusing on decoding strategies?}\yjc{argee that other factors also affect data quality, we only study decoding strategy here because of the unnatural finding in \S4.3.2. maybe add experiments on other factors to Appendix later}
}
\label{tab:quality}
\vspace{-2mm}
\end{table}

==> tabs/data_scale.tex <==
% \begin{table}[t]
% \scalebox{0.75}{
% \begin{tabular}{lll|ccc}
% \toprule
% \multicolumn{1}{c}{\textbf{Setting}} & \textbf{TAM} & \textbf{Scale} & \textbf{IMDB} & \textbf{SQuAD} & \textbf{QNLI} \\
% \hline
% \multirow{2}{*}{\textit{\textsc{Supervised}}} & LSTM & 1x & 84.60 & 41.86/57.22 & 69.00 \\
%  & DistilBERT & 1x & 87.24 & 76.28/84.67 & 88.05 \\
%  \hline
% \textit{\textsc{Prompting}} & - & 0x & 80.64 & 4.61/13.32 & 60.60 \\
% \hline
% \multirow{6}{*}{\textit{\textsc{ZeroGen}}} & \multirow{3}{*}{LSTM} & 0.5x & 53.20 & \textbf{7.71}/12.11 & 52.39 \\
%  &  & 1x & 59.30 & \textbf{8.57}/\textbf{13.63} & 51.16 \\
%  &  & 2x & 69.10 & \textbf{9.73}/\textbf{15.12} & 51.22 \\
%  \cline{2-6}
%  & \multirow{3}{*}{DistilBERT} & 0.5x & 80.05 & \textbf{20.47}/\textbf{27.20} & \textbf{69.80} \\
%  &  & 1x & \textbf{80.90} & \textbf{23.63}/\textbf{29.95} & \textbf{70.55} \\
%  &  & 2x & \textbf{81.60} & \textbf{25.25}/\textbf{31.50} & \textbf{71.19} \\
%  \bottomrule
% \end{tabular}}
% \caption{Comparison of different scale of synthetic dataset. We use GPT2-XL as the PLM for both \textsc{Prompting} and \textsc{ZeroGen} frameworks. }
% \label{tab:scale}
% \end{table}

\begin{table}[t]
\centering
\scalebox{0.7}{
\begin{tabular}{lll|ccc}
\toprule
\multicolumn{1}{c}{\textbf{Setting}} & \textbf{TAM} & \textbf{Scale} & \textbf{IMDB} & \textbf{SQuAD} & \textbf{QNLI} \\
\hline
\multirow{2}{*}{\textit{\textsc{Supervised}}} & LSTM & 1x & 84.60 & 41.86/57.22 & 69.00 \\
 & DistilBERT & 1x & 87.24 & 76.28/84.67 & 88.05 \\
 \hline
\textit{\textsc{Prompting}} & - & 0x & 80.64 & 4.61/13.32 & 60.60 \\
\hline
\multirow{6}{*}{\textit{\textsc{ZeroGen}}} & \multirow{3}{*}{LSTM} & 0.5x & 53.20 & \cc {7.71}/12.11 & {50.05} \\
 &  & 1x & 59.30 & \cc {8.57}/{13.63} & 51.16 \\
 &  & 2x & \textbf{69.10} & \cc \textbf{9.73}/\textbf{15.12} & \textbf{52.26} \\
 \cline{2-6}
 & \multirow{3}{*}{DistilBERT} & 0.5x & 80.05 & \cc {20.47}/{27.20} & \cc {69.80} \\
 &  & 1x & \cc {80.90} & \cc {23.63}/{29.95} & \cc {70.55} \\
 &  & 2x & \cc \textbf{81.60} & \cc \textbf{25.25}/\textbf{31.50} & \cc \textbf{71.19} \\
 \bottomrule
\end{tabular}}
\caption{Comparison of different scale of synthetic dataset. We use GPT2-XL as the PLM for both \textsc{Prompting} and \textsc{ZeroGen} frameworks. Under different scales of dataset, best results are \textbf{bolded}.}
\label{tab:scale}
\end{table}

==> tabs/notation.tex <==

\begin{table*}[t]
\centering
\scalebox{0.8}{
\begin{tabular}{l|llp{10cm}}
\toprule
 & \textbf{Dataset} & \textbf{Dataset Generation} & \textbf{Example} \\ 
 \hline
\multirow{2}{*}{\textbf{TC}} & \multirow{2}{*}{$\{(X, y)\}$} & \multirow{2}{*}{$X \sim P(X|f_{prompt}(y))$} & $\operatorname{Des}(y)$: \{positive, negative\} \\
 &  &  & $f_{prompt}$: The movie review in <$\operatorname{Des}(y)$> sentiment is: " \\ 
 \hline
\multirow{2}{*}{\textbf{NLI}} & \multirow{2}{*}{$\{(P, H, y)\}$} & {\multirow{2}{*}{$H \sim P(H|f_{prompt}(y, P))$}} & $\operatorname{Des}(y)$: \{correct, wrong\} \\
 &  &  & $f_{prompt}$: "<$P$>"\textbackslash{}nBased on the above description, the following sentence is definitely <$\operatorname{Des}(y)$>: " \\ 
 \hline
\textbf{QA} & $\{(Q, C, A)\}$ & $Q\sim P(Q|f_{prompt}(C,A))$ & $f_{prompt}$: The context is: "<$Q$>" \textbackslash{}n"<$A$>" is the answer of the following question: " \\ 
\bottomrule
\end{tabular}}
\caption{Notation and example of dataset generation methods for three tasks with our \proposed\ framework. $\operatorname{Des}(y)$: description of label $y$.}
\label{tab:approach}
\end{table*}
